UIVNAV: Underwater Information-driven Vision-based Navigation via Imitation Learning

Autonomous navigation in the underwater environment is challenging due to limited visibility, dynamic changes, and the lack of a cost-efficient accurate localization system. We introduce UIVNav, a novel end-to-end underwater navigation solution designed to drive robots over Objects of Interest (OOI) while avoiding obstacles, without relying on localization. UIVNav uses imitation learning and is inspired by the navigation strategies used by human divers who do not rely on localization. UIVNav consists of the following phases: (1) generating an intermediate representation (IR), and (2) training the navigation policy based on human-labeled IR. By training the navigation policy on IR instead of raw data, the second phase is domain-invariant -- the navigation policy does not need to be retrained if the domain or the OOI changes. We show this by deploying the same navigation policy for surveying two different OOIs, oyster and rock reefs, in two different domains, simulation, and a real pool. We compared our method with complete coverage and random walk methods which showed that our method is more efficient in gathering information for OOIs while also avoiding obstacles. The results show that UIVNav chooses to visit the areas with larger area sizes of oysters or rocks with no prior information about the environment or localization. Moreover, a robot using UIVNav compared to complete coverage method surveys on average 36% more oysters when traveling the same distances. We also demonstrate the feasibility of real-time deployment of UIVNavin pool experiments with BlueROV underwater robot for surveying a bed of oyster shells.

==> sections/ack.tex <==
\section*{ACKNOWLEDGMENT}
We would like to thank Tianchen Liu and Kaustubh Sandeep Joshi from the University of Maryland for helping us with various tasks. This work was supported by USDA NIFA sustainable agriculture system
program under award number 20206801231805.

==> sections/reviews.tex <==
Reviewer 5 of ICRA 2024 submission 1116

Comments to the author
======================

Paper Summary:
This paper presents a novel end-to-end underwater
navigation scheme that trains navigation strategies by
generating intermediate representation (IR) and IR based on
artificial markers. The authors demonstrate this through
simulations and experiments, being able to avoid obstacles
and not relying on localization, and that the trained
strategies are able to adapt to different environments
without the need to retrain the navigation strategies. It
is an interesting research work for navigation in
underwater environments.

Paper Strengths:
The idea of training navigation strategies in a
domain-invariant manner to reduce the need for retraining
to adapt to new environments is significant and can help
develop additional functionality for underwater navigation.
The essay is well-structured, logical, and readable.


Paper Weaknesses:
Noting that the validation experiments showed that the
underwater robot was able to navigate to avoid obstacles,
has this been considered in terms of how the size of the
obstacles would affect navigation, e.g. in extreme cases
the obstacles were very high?

What are the advantages of training a strategy by training
it on IR rather than on raw data?

Noting that the authors are looking at static areas, such
as oysters, as areas of interest, has it been considered
that the OOI is a dynamic area, such as a school of
swimming fish?

There are also some grammatical errors in the writing of
the article that need to be checked and corrected, such as
in the last paragraph of the second section where it should
be "... strategy that using IR..." in the last paragraph of
the second section, instead of "... strategy which using
IR...".


Comments on the Video Attachment
================================

It contributes to helping the reader visualize more of the
work done in the article.


Reviewer 4 of ICRA 2024 submission 1116

Comments to the author
======================

The paper proposes to tackle the challenge of navigating
underwater in an unknown environment and imitate the
strategies adopted by human divers. The results shown are
quite promising and cost and time-efficient. The following
information should be provided to make it more useful to
the readers:  
- what type of camera will be required if the images are
not visible underwater
- how this planner will accommodate the dynamic obstacles
(such as moving fish or mammals)
- Not sure whether the time for exploration in Fig 4 was
the same for all strategies or different times were taken.
If different times had elapsed to cover the areas then how
this approach is efficient considering the limited battery
power available in robots.
- if the results needed only to control the yaw and pitch
of the robots then why 6 degrees of freedom are required -
please explain
- how 1500 is in equation 2 - not explained
- whether this approach can be used as a local planner in a
swarm and how this can be achieved using the proposed
algorithms and what will be the benefits
- The paper fails to indicate the details of the
technologies used in Imitation and depth estimation -
Please elaborate
- The future work indicated in the paper is quite vague.
For example - Soanr detection will generate a large amount
of data and will be difficult to apply in real-time with
the same setup. The future work should include how this
technology can be improved further to work with global
localization, in swarm and how the data can be transferred
in cooperation 


Comments on the Video Attachment
================================

Thanks for sharing a video showing the effectiveness of the
approach

